Thermal Chameleon: Task-Adaptive Tone-mapping for Radiometric Thermal-Infrared images

Thermal Infrared (TIR) imaging provides robust perception for navigating in challenging outdoor environments but faces issues with poor texture and low image contrast due to its 14/16-bit format. Conventional methods utilize various tone-mapping methods to enhance contrast and photometric consistency of TIR images, however, the choice of tone-mapping is largely dependent on knowing the task and temperature dependent priors to work well. In this paper, we present Thermal Chameleon Network (TCNet), a task-adaptive tone-mapping approach for RAW 14-bit TIR images. Given the same image, TCNet tone-maps different representations of TIR images tailored for each specific task, eliminating the heuristic image rescaling preprocessing and reliance on the extensive prior knowledge of the scene temperature or task-specific characteristics. TCNet exhibits improved generalization performance across object detection and monocular depth estimation, with minimal computational overhead and modular integration to existing architectures for various tasks. Project Page: https://github.com/donkeymouse/ThermalChameleon

==> tables/dataset-survey.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[h]
\centering
\caption{List of recent thermal infrared dataset benchmarks}
\label{tab:dataset-survey}
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{cccc}
\hline \hline
Name             & Task                                                             & Radiometric? & \begin{tabular}[c]{@{}c@{}}Camera Offset\\ Parameters\end{tabular} \\ \hline
OdomBeyondVision \cite{li2022odombeyondvision} & Odometry                                                         & Yes          & No                                                                 \\
VIVID \cite{lee2022vivid++}            & Odometry/Depth                                                   & Yes          & Yes                                                                \\
MS2 \cite{shin2023cvpr}              & Odometry/Depth                                                   & Yes          & Yes                                                                \\
LTIR \cite{berg2015tracking}             & Tracking                                                         & Yes          & No                                                                 \\
CART \cite{lee2024cart}             & \begin{tabular}[c]{@{}c@{}}Semantic \\ Segmentation\end{tabular} & No           & No                                                                 \\
PST900 \cite{shivakumar2020pst900}           & \begin{tabular}[c]{@{}c@{}}Semantic \\ Segmentation\end{tabular} & No           & No                                                                 \\
STheReO \cite{yun2022sthereo}         & Odometry                                                         & Yes          & Yes                                                                \\
NSVPS \cite{carmichael2024nsvps}            & Odometry                                                         & Yes          & No                                                                 \\
FLIR-ADAS \cite{fliradas}        & \begin{tabular}[c]{@{}c@{}}Object \\ Detection\end{tabular}      & Yes          & No                                                                 \\ \hline \hline
\end{tabular}%
}
\end{table}

==> tables/naive-blocks.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[h]
\centering
\caption{Object detection results with popular backbone blocks}
\label{naive-blocks}
\resizebox{0.5\columnwidth}{!}{%
\begin{tabular}{crrrrrr}
\hline
Augmentation    & \multicolumn{1}{c}{mAP} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}mAP\\ @0.5\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}mAP\\ @0.75\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}mAP\\ @small\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}mAP\\ @medium\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}mAP\\ @large\end{tabular}} \\ \hline
UNet \cite{ronneberger2015unet}            & 0.532                   & 0.788                                                                  & 0.566                                                                   & 0.447                                                                    & 0.728                                                                     & 0.724                                                                    \\
Resblock \cite{he2016resnet}        & 0.477                   & 0.734                                                                  & 0.518                                                                   & 0.403                                                                    & 0.651                                                                     & 0.581                                                                    \\
NLNet \cite{wang2018nlnet} \cite{}           & 0.491                   & 0.754                                                                  & 0.529                                                                   & 0.421                                                                    & 0.656                                                                     & 0.589                                                                    \\
SENet \cite{senet}           & 0.518                   & 0.801                                                                  & 0.555                                                                   & 0.434                                                                    & 0.701                                                                     & 0.746                                                                    \\
Xu et. al. \cite{xu2023toward} & 0.529                   & 0.81                                                                   & 0.572                                                                   & 0.433                                                                    & 0.715                                                                     & 0.732                                                                    \\
TCNet           & \textbf{0.56}           & \textbf{0.838}                                                         & \textbf{0.605}                                                          & \textbf{0.478}                                                           & \textbf{0.734}                                                            & \textbf{0.77}                                                            \\ \hline
\end{tabular}%
}
\end{table}

==> tables/obj_det_table_channel_valley.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Ablation study for varying the number of input thermal embedding channels for detection on STheReO dataset.}
\label{tab:channel-valley}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccc}
\hline \hline
\multicolumn{7}{c}{Dataset: STheReO-Valley}                                                                                                   \\ \hline \hline
\multicolumn{7}{c}{RetinaNet}                                                                                                            \\ \hline \hline
\multicolumn{1}{c|}{Compression}         & mAP           & \begin{tabular}[c]{@{}c@{}}mAP\\ @0.5\end{tabular}       & \begin{tabular}[c]{@{}c@{}}mAP\\ @0.75\end{tabular}      & \begin{tabular}[c]{@{}c@{}}mAP\\ @small\end{tabular}     & \begin{tabular}[c]{@{}c@{}}mAP\\ @medium\end{tabular}    & \begin{tabular}[c]{@{}c@{}}mAP\\ @large\end{tabular}     \\ \hline 
\multicolumn{1}{c|}{$3 \rightarrow 3 $}  & 32.2          & 59.4          & 31.7          & 10.3          & 42.1          & 56.8          \\
\multicolumn{1}{c|}{$8 \rightarrow 3 $}  & \textbf{36.1} & \textbf{62.0} & \textbf{37.3} & \textbf{12.6} & \textbf{46.8} & \textbf{66.6} \\
\multicolumn{1}{c|}{$10 \rightarrow 3 $} & 34.2          & 59.0          & 35.5          & 11.6          & 44.0          & 61.9          \\
\multicolumn{1}{c|}{$12 \rightarrow 3 $} & 33.8          & 58.5          & 34.0          & 10.3          & 45.4          & 61.3          \\ \hline \hline
\multicolumn{7}{c}{YOLO-X}                                                                                                               \\ \hline \hline
\multicolumn{1}{c|}{Compression}         & mAP           & \begin{tabular}[c]{@{}c@{}}mAP\\ @0.5\end{tabular}       & \begin{tabular}[c]{@{}c@{}}mAP\\ @0.75\end{tabular}      & \begin{tabular}[c]{@{}c@{}}mAP\\ @small\end{tabular}     & \begin{tabular}[c]{@{}c@{}}mAP\\ @medium\end{tabular}    & \begin{tabular}[c]{@{}c@{}}mAP\\ @large\end{tabular}     \\ \hline
\multicolumn{1}{c|}{$3 \rightarrow 3 $}  & 47.2          & 79.7          & 48.1          & 24.5          & 56.1          & 74.2          \\
\multicolumn{1}{c|}{$8 \rightarrow 3 $}  & 47.9          & \textbf{81.3} & 49.2          & 24.8          & 57.0          & \textbf{76.4} \\
\multicolumn{1}{c|}{$10 \rightarrow 3 $} & 47.5          & 80.0          & 48.6          & 24.4          & 56.6          & 75.3          \\
\multicolumn{1}{c|}{$12 \rightarrow 3 $} & \textbf{48.3} & 81.0          & \textbf{50.0} & \textbf{24.9} & \textbf{57.6} & 75.7          \\ \hline \hline
\multicolumn{7}{c}{Sparse RCNN}                                                                                                          \\ \hline \hline
\multicolumn{1}{c|}{Compression}         & mAP           & \begin{tabular}[c]{@{}c@{}}mAP\\ @0.5\end{tabular}       & \begin{tabular}[c]{@{}c@{}}mAP\\ @0.75\end{tabular}      & \begin{tabular}[c]{@{}c@{}}mAP\\ @small\end{tabular}     & \begin{tabular}[c]{@{}c@{}}mAP\\ @medium\end{tabular}    & \begin{tabular}[c]{@{}c@{}}mAP\\ @large\end{tabular}     \\ \hline
\multicolumn{1}{c|}{$3 \rightarrow 3 $}  & 39.2          & 70.8          & \textbf{38.4} & 18.7          & 47.7          & \textbf{69.1} \\
\multicolumn{1}{c|}{$8 \rightarrow 3 $}  & 37.8          & 70.5          & 35.1          & 17.9          & 48.9          & 65.3          \\
\multicolumn{1}{c|}{$10 \rightarrow 3 $} & 37.1          & 69.8          & 34.8          & 15.3          & 47.3          & 66.2          \\
\multicolumn{1}{c|}{$12 \rightarrow 3 $} & \textbf{39.5} & \textbf{73.2} & 38.2          & \textbf{18.8} & \textbf{49.4} & 63.5          \\ \hline \hline
\end{tabular}%
}

\end{table}

==> tables/pose-estimation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Pose estimation results. Best results highlighted in \textbf{bold}; Second best in \underline{underlines}.}
\label{tab:pose-estimation}
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{c|cc|cc}
\hline \hline
\multirow{2}{*}{Baselines} & \multicolumn{2}{c|}{VIVID}        & \multicolumn{2}{c}{MS2}           \\ \cline{2-5} 
                           & ATE             & RE              & ATE             & RE              \\ \hline
RAW                        & 0.1034          & 0.0320           & 0.7285          & 0.0145          \\
Minmax                     & 0.0715          & 0.0284          & 0.4988          & 0.0188          \\
Clip                       & 0.0885          & 0.0298          & 0.5655          & 0.0335          \\
HE                         & \underline{0.0546}          & 0.0287          & \textbf{0.2281} & 0.0279          \\
Fieldscale                 & 0.0982          & 0.0679          & 0.6263          & 0.4342          \\
Shin                       & 0.0571          & \underline{0.0280}           & 0.2878          & 0.0201          \\ \hline
TE(3)                      & 0.0688          & 0.0282          & 0.3836          & 0.0320          \\
TE(10)                     & 0.0669          & 0.0342          & 0.2839          & \textbf{0.0118} \\
TCNet                      & \textbf{0.0534} & \textbf{0.0269} & \underline{0.2399}          & \underline{0.0142}          \\ \hline \hline
\end{tabular}%
}
\end{table}
